Self-Adaptation and Secure Information Flow in Multiparty Structured Communications: A Unified Perspective

We present initial results on a comprehensive model of structured communications, in which self- adaptation and security concerns are jointly addressed. More specifically, we propose a model of self-adaptive, multiparty communications with secure information flow guarantees. In this model, security violations occur when processes attempt to read or write messages of inappropriate security levels within directed exchanges. Such violations trigger adaptation mechanisms that prevent the violations to occur and/or to propagate their effect in the choreography. Our model is equipped with local and global mechanisms for reacting to security violations; type soundness results ensure that global protocols are still correctly executed, while the system adapts itself to preserve security.

==> eptcsdata.tex <==
\providecommand{\firstpage}{9}
\providecommand{\publicationstatus}{Marco Carbone (Ed.): Third Workshop on\\
Behavioural Types (BEAT 2014)\\
EPTCS 162, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.162.2}{10.4204/EPTCS.162.2}}

